Recent Developments and Future Challenges in Medical Mixed Reality

Mixed Reality (MR) is of increasing interest within technology-driven modern medicine but is not yet used in everyday practice. This situation is changing rapidly, however, and this paper explores the emergence of MR technology and the importance of its utility within medical applications. A classification of medical MR has been obtained by applying an unbiased text mining method to a database of 1,403 relevant research papers published over the last two decades. The classification results reveal a taxonomy for the development of medical MR research during this period as well as suggesting future trends. We then use the classification to analyse the technology and applications developed in the last five years. Our objective is to aid researchers to focus on the areas where technology advancements in medical MR are most needed, as well as providing medical practitioners with a useful source of reference.

==> Biographies.tex <==
% biography section
% 
% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:


\begin{IEEEbiographynophoto}{Long Chen}
Long Chen graduated from the Dalian University of Technology, China, in 2013, and received a Masters degree in Physics and Engineer in Medicine with distinction from the University College London, U.K. in 2014. After graduation, he worked for GE Healthcare and Toshiba Medical System for a gap year. He is now a PhD student at Bournemouth University researching Augmented Reality in Medicine. His research interests are AR/VR in medicine, medical imaging and computer vision.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Thomas W Day}
is a PhD Student researching the use of Augmented Reality in Medicine at the University of Chester under the supervision of Prof. Nigel W John. He previously studied Computer Science at Bangor University in the United Kingdom where he obtained a first class degree.

While at Bangor, he interned as a researcher for the Biomedical Research Unit for Advanced Medical Imaging and Visualization looking into the medical applications of virtual environments and haptic devices.
\end{IEEEbiographynophoto}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{Wen Tang, Member of EG, Member of IEEE}is a Professor of Creative Technology at the Bournemouth University, UK. She is Head of Research of Creative Technology Department and leads the Centre for Games and Music Technology Research at the university. Wen Tang's research expertise is in 3D computer graphics and games technology, specifically 3D physically based computer graphics algorithms and interactive techniques for digital games and virtual environments. Her research work is both fundamental (e.g. 3D computational algorithms with real time performance), technical (e.g.3D virtual reality system design and development) and applied (e.g. applications of games and virtual reality techniques in health, training and education). She a principal investigator for several 3D computer simulations systems, for example, a surgical training system for Minimally Invasive procedures, an exercise gaming platform for delivering high intensity level of physical activity to improve health and wellbeing of people.

\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Nigel W John FEG FLSW}
 is a Professor of Computer Science at the University of Chester in the United Kingdom where he has established a new Medical Graphics Research group. Previously he was responsible for research activities in visualization and computer graphics at Bangor University and the University of Manchester. He was also a co-Director and founder of the Welsh Assembly Government funded Research Institute of Visual Computing, and Director and founder of the Biomedical Research Unit for Advanced Medical Imaging and Visualization. 
 
 Prof. John has thirty years of research experience and has been awarded grants for many projects involving high performance visualisation, haptics, augmented reality and virtual environments. He has over 100 publications in peer reviewed conferences and journals in the field. In 2006, he received the Twelfth Annual Satava Award for accomplishments to the field of computer graphics and medical visualization. Each year the award is presented to an individual or group who demonstrate unique vision and commitment to the improvement of medicine with the use of advanced technology. Current research interests are focused on the application of augmented reality technologies to medical applications.

 Prof John is an elected Fellow of the Eurographics Association and was co-chair of the EG2001 and EG2008 conferences, and formerly the chair of the Eurographics Professional Board. He is a Fellow of the Learned Society of Wales (elected in 2014). In 2013 he became a Churchill Travelling Fellow. In 2016 he became a Fellow of the Higher Education Academy.


\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

